KnowCoder-V2: Deep Knowledge Analysis

Deep knowledge analysis tasks always involve the systematic extraction and association of knowledge from large volumes of data, followed by logical reasoning to discover insights. However, to solve such complex tasks, existing deep research frameworks face three major challenges: 1) They lack systematic organization and management of knowledge; 2) They operate purely online, making it inefficient for tasks that rely on shared and large-scale knowledge; 3) They cannot perform complex knowledge computation, limiting their abilities to produce insightful analytical results. Motivated by these, in this paper, we propose a \textbf{K}nowledgeable \textbf{D}eep \textbf{R}esearch (\textbf{KDR}) framework that empowers deep research with deep knowledge analysis capability. Specifically, it introduces an independent knowledge organization phase to preprocess large-scale, domain-relevant data into systematic knowledge offline. Based on this knowledge, it extends deep research with an additional kind of reasoning steps that perform complex knowledge computation in an online manner. To enhance the abilities of LLMs to solve knowledge analysis tasks in the above framework, we further introduce \textbf{\KCII}, an LLM that bridges knowledge organization and reasoning via unified code generation. For knowledge organization, it generates instantiation code for predefined classes, transforming data into knowledge objects. For knowledge computation, it generates analysis code and executes on the above knowledge objects to obtain deep analysis results. Experimental results on more than thirty datasets across six knowledge analysis tasks demonstrate the effectiveness of \KCII. Moreover, when integrated into the KDR framework, \KCII can generate high-quality reports with insightful analytical results compared to the mainstream deep research framework.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> reference.tex <==
\begin{thebibliography}{77}
    \providecommand{\natexlab}[1]{#1}
    \providecommand{\url}[1]{\texttt{#1}}
    \expandafter\ifx\csname urlstyle\endcsname\relax
      \providecommand{\doi}[1]{doi: #1}\else
      \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi
    
    \bibitem[Achiam et~al.(2023)Achiam, Adler, Agarwal, Ahmad, Akkaya, Aleman,
      Almeida, Altenschmidt, Altman, Anadkat, et~al.]{achiam2023gpt}
    Josh Achiam, Steven Adler, Sandhini Agarwal, Lama Ahmad, Ilge Akkaya,
      Florencia~Leoni Aleman, Diogo Almeida, Janko Altenschmidt, Sam Altman,
      Shyamal Anadkat, et~al.
    \newblock Gpt-4 technical report.
    \newblock \emph{arXiv preprint arXiv:2303.08774}, 2023.
    
    \bibitem[Alzubi et~al.(2025)Alzubi, Brooks, Chiniya, Contente, von Gerlach,
      Irwin, Jiang, Kaz, Nguyen, Oh, et~al.]{alzubi2025open}
    Salaheddin Alzubi, Creston Brooks, Purva Chiniya, Edoardo Contente, Chiara von
      Gerlach, Lucas Irwin, Yihan Jiang, Arda Kaz, Windsor Nguyen, Sewoong Oh,
      et~al.
    \newblock Open deep search: Democratizing search with open-source reasoning
      agents.
    \newblock \emph{arXiv preprint arXiv:2503.20201}, 2025.
    
    \bibitem[Asai et~al.(2023)Asai, Wu, Wang, Sil, and Hajishirzi]{asai2023self}
    Akari Asai, Zeqiu Wu, Yizhong Wang, Avirup Sil, and Hannaneh Hajishirzi.
    \newblock Self-rag: Learning to retrieve, generate, and critique through
      self-reflection.
    \newblock In \emph{The Twelfth International Conference on Learning
      Representations}, 2023.
    
    \bibitem[Bansal et~al.(2014)Bansal, Burkett, De~Melo, and
      Klein]{bansal2014structured}
    Mohit Bansal, David Burkett, Gerard De~Melo, and Dan Klein.
    \newblock Structured learning for taxonomy induction with belief propagation.
    \newblock In \emph{ACL}, pp.\  1041--1051, 2014.
    
    \bibitem[Bordea et~al.(2016)Bordea, Lefever, and Buitelaar]{bordea2016semeval}
    Georgeta Bordea, Els Lefever, and Paul Buitelaar.
    \newblock Semeval-2016 task 13: Taxonomy extraction evaluation (texeval-2).
    \newblock In \emph{Proceedings of the 10th international workshop on semantic
      evaluation (semeval-2016)}, pp.\  1081--1091, 2016.
    
    \bibitem[Chen et~al.(2025)Chen, Li, Sun, Zhou, Zhu, Yang, Zhou, Chen, Wang,
      Pan, et~al.]{chen2025learning}
    Mingyang Chen, Tianpeng Li, Haoze Sun, Yijie Zhou, Chenzheng Zhu, Fan Yang,
      Zenan Zhou, Weipeng Chen, Haofen Wang, Jeff~Z Pan, et~al.
    \newblock Learning to reason with search for llms via reinforcement learning.
    \newblock \emph{arXiv preprint arXiv:2503.19470}, 2025.
    
    \bibitem[Cowie \& Lehnert(1996)Cowie and Lehnert]{cowie1996information}
    Jim Cowie and Wendy Lehnert.
    \newblock Information extraction.
    \newblock \emph{Communications of the ACM}, 39\penalty0 (1):\penalty0 80--91,
      1996.
    
    \bibitem[Edge et~al.(2024)Edge, Trinh, Cheng, Bradley, Chao, Mody, Truitt,
      Metropolitansky, Ness, and Larson]{edge2024local}
    Darren Edge, Ha~Trinh, Newman Cheng, Joshua Bradley, Alex Chao, Apurva Mody,
      Steven Truitt, Dasha Metropolitansky, Robert~Osazuwa Ness, and Jonathan
      Larson.
    \newblock From local to global: A graph rag approach to query-focused
      summarization.
    \newblock \emph{arXiv preprint arXiv:2404.16130}, 2024.
    
    \bibitem[Gao et~al.(2021)Gao, Yao, and Chen]{gao2021simcse}
    Tianyu Gao, Xingcheng Yao, and Danqi Chen.
    \newblock Simcse: Simple contrastive learning of sentence embeddings.
    \newblock In \emph{Proceedings of the 2021 Conference on Empirical Methods in
      Natural Language Processing}, pp.\  6894. Association for Computational
      Linguistics, 2021.
    
    \bibitem[Guan et~al.(2024)Guan, Man, Chen, Yao, Hu, Zhu, Smith, Lim, and
      Yue]{guan2024findvehicle}
    Runwei Guan, Ka~Lok Man, Feifan Chen, Shanliang Yao, Rongsheng Hu, Xiaohui Zhu,
      Jeremy Smith, Eng~Gee Lim, and Yutao Yue.
    \newblock Findvehicle and vehiclefinder: a ner dataset for natural
      language-based vehicle retrieval and a keyword-based cross-modal vehicle
      retrieval system.
    \newblock \emph{Multimedia Tools and Applications}, 83\penalty0 (8):\penalty0
      24841--24874, 2024.
    
    \bibitem[Gui et~al.(2024{\natexlab{a}})Gui, Yuan, Ye, Zhang, Sun, Liang, and
      Chen]{gui2024iepile}
    Honghao Gui, Lin Yuan, Hongbin Ye, Ningyu Zhang, Mengshu Sun, Lei Liang, and
      Huajun Chen.
    \newblock Iepile: Unearthing large-scale schema-based information extraction
      corpus.
    \newblock \emph{arXiv preprint arXiv:2402.14710}, 2024{\natexlab{a}}.
    
    \bibitem[Gui et~al.(2024{\natexlab{b}})Gui, Yuan, Ye, Zhang, Sun, Liang, and
      Chen]{gui2024iepileunearthinglargescaleschemabased}
    Honghao Gui, Lin Yuan, Hongbin Ye, Ningyu Zhang, Mengshu Sun, Lei Liang, and
      Huajun Chen.
    \newblock Iepile: Unearthing large-scale schema-based information extraction
      corpus, 2024{\natexlab{b}}.
    \newblock URL \url{https://arxiv.org/abs/2402.14710}.
    
    \bibitem[Guo et~al.(2025)Guo, Yang, Zhang, Song, Zhang, Xu, Zhu, Ma, Wang, Bi,
      et~al.]{guo2025deepseek}
    Daya Guo, Dejian Yang, Haowei Zhang, Junxiao Song, Ruoyu Zhang, Runxin Xu,
      Qihao Zhu, Shirong Ma, Peiyi Wang, Xiao Bi, et~al.
    \newblock Deepseek-r1: Incentivizing reasoning capability in llms via
      reinforcement learning.
    \newblock \emph{arXiv preprint arXiv:2501.12948}, 2025.
    
    \bibitem[Guo et~al.(2023)Guo, Li, Jin, Liu, Zeng, Liu, Li, Yang, Bai, Guo, and
      Cheng]{guo2023retrievalaugmentedcodegenerationuniversal}
    Yucan Guo, Zixuan Li, Xiaolong Jin, Yantao Liu, Yutao Zeng, Wenxuan Liu, Xiang
      Li, Pan Yang, Long Bai, Jiafeng Guo, and Xueqi Cheng.
    \newblock Retrieval-augmented code generation for universal information
      extraction, 2023.
    \newblock URL \url{https://arxiv.org/abs/2311.02962}.
    
    \bibitem[Gurulingappa et~al.(2012)Gurulingappa, Rajput, Roberts, Fluck,
      Hofmann-Apitius, and Toldo]{ADEcorpus_DATASET}
    Harsha Gurulingappa, Abdul~Mateen Rajput, Angus Roberts, Juliane Fluck, Martin
      Hofmann-Apitius, and Luca Toldo.
    \newblock Development of a benchmark corpus to support the automatic extraction
      of drug-related adverse effects from medical case reports.
    \newblock \emph{Journal of Biomedical Informatics}, 45\penalty0 (5):\penalty0
      885--892, 2012.
    \newblock ISSN 1532-0464.
    \newblock \doi{https://doi.org/10.1016/j.jbi.2012.04.008}.
    \newblock URL
      \url{https://www.sciencedirect.com/science/article/pii/S1532046412000615}.
    \newblock Text Mining and Natural Language Processing in Pharmacogenomics.
    
    \bibitem[He et~al.(2021)He, Lan, Jiang, Zhao, and Wen]{NSM}
    Gaole He, Yunshi Lan, Jing Jiang, Wayne~Xin Zhao, and Ji{-}Rong Wen.
    \newblock Improving multi-hop knowledge base question answering by learning
      intermediate supervision signals.
    \newblock In Liane Lewin{-}Eytan, David Carmel, Elad Yom{-}Tov, Eugene
      Agichtein, and Evgeniy Gabrilovich (eds.), \emph{{WSDM} '21, The Fourteenth
      {ACM} International Conference on Web Search and Data Mining, Virtual Event,
      Israel, March 8-12, 2021}, pp.\  553--561. {ACM}, 2021.
    \newblock \doi{10.1145/3437963.3441753}.
    \newblock URL \url{https://doi.org/10.1145/3437963.3441753}.
    
    \bibitem[He et~al.(2024)He, Tian, Sun, Chawla, Laurent, LeCun, Bresson, and
      Hooi]{he2024g}
    Xiaoxin He, Yijun Tian, Yifei Sun, Nitesh Chawla, Thomas Laurent, Yann LeCun,
      Xavier Bresson, and Bryan Hooi.
    \newblock G-retriever: Retrieval-augmented generation for textual graph
      understanding and question answering.
    \newblock \emph{Advances in Neural Information Processing Systems},
      37:\penalty0 132876--132907, 2024.
    
    \bibitem[Hendrickx et~al.(2010)Hendrickx, Kim, Kozareva, Nakov,
      {\'O}~S{\'e}aghdha, Pad{\'o}, Pennacchiotti, Romano, and
      Szpakowicz]{hendrickx-etal-2010-semeval}
    Iris Hendrickx, Su~Nam Kim, Zornitsa Kozareva, Preslav Nakov, Diarmuid
      {\'O}~S{\'e}aghdha, Sebastian Pad{\'o}, Marco Pennacchiotti, Lorenza Romano,
      and Stan Szpakowicz.
    \newblock {S}em{E}val-2010 task 8: Multi-way classification of semantic
      relations between pairs of nominals.
    \newblock In Katrin Erk and Carlo Strapparava (eds.), \emph{Proceedings of the
      5th International Workshop on Semantic Evaluation}, pp.\  33--38, Uppsala,
      Sweden, July 2010. Association for Computational Linguistics.
    \newblock URL \url{https://aclanthology.org/S10-1006}.
    
    \bibitem[Hu et~al.(2021)Hu, Shen, Wallis, Allen-Zhu, Li, Wang, Wang, and
      Chen]{hu2021loralowrankadaptationlarge}
    Edward~J. Hu, Yelong Shen, Phillip Wallis, Zeyuan Allen-Zhu, Yuanzhi Li, Shean
      Wang, Lu~Wang, and Weizhu Chen.
    \newblock Lora: Low-rank adaptation of large language models, 2021.
    \newblock URL \url{https://arxiv.org/abs/2106.09685}.
    
    \bibitem[Hui et~al.(2024)Hui, Yang, Cui, Yang, Liu, Zhang, Liu, Zhang, Yu, Lu,
      Dang, Fan, Zhang, Yang, Men, Huang, Zheng, Miao, Quan, Feng, Ren, Ren, Zhou,
      and Lin]{hui2024qwen25codertechnicalreport}
    Binyuan Hui, Jian Yang, Zeyu Cui, Jiaxi Yang, Dayiheng Liu, Lei Zhang, Tianyu
      Liu, Jiajun Zhang, Bowen Yu, Keming Lu, Kai Dang, Yang Fan, Yichang Zhang,
      An~Yang, Rui Men, Fei Huang, Bo~Zheng, Yibo Miao, Shanghaoran Quan, Yunlong
      Feng, Xingzhang Ren, Xuancheng Ren, Jingren Zhou, and Junyang Lin.
    \newblock Qwen2.5-coder technical report, 2024.
    \newblock URL \url{https://arxiv.org/abs/2409.12186}.
    
    \bibitem[Jiang et~al.(2023{\natexlab{a}})Jiang, Zhou, Dong, Ye, Zhao, and
      Wen]{structgpt}
    Jinhao Jiang, Kun Zhou, Zican Dong, Keming Ye, Wayne~Xin Zhao, and Ji-Rong Wen.
    \newblock Structgpt: A general framework for large language model to reason
      over structured data, 2023{\natexlab{a}}.
    
    \bibitem[Jiang et~al.(2023{\natexlab{b}})Jiang, Yao, Wang, and
      Sun]{jiang2023single}
    Song Jiang, Qiyue Yao, Qifan Wang, and Yizhou Sun.
    \newblock A single vector is not enough: Taxonomy expansion via box embeddings.
    \newblock In \emph{Proceedings of the ACM Web Conference 2023}, pp.\
      2467--2476, 2023{\natexlab{b}}.
    
    \bibitem[Jin et~al.(2025)Jin, Zeng, Yue, Wang, Zamani, and Han]{jin2025search}
    Bowen Jin, Hansi Zeng, Zhenrui Yue, Dong Wang, Hamed Zamani, and Jiawei Han.
    \newblock Search-r1: Training llms to reason and leverage search engines with
      reinforcement learning.
    \newblock \emph{arXiv preprint arXiv:2503.09516}, 2025.
    
    \bibitem[Kocaman \& Talby(2020)Kocaman and Talby]{DBLP:conf/icpr/KocamanT20}
    Veysel Kocaman and David Talby.
    \newblock Biomedical named entity recognition at scale.
    \newblock In Alberto~Del Bimbo, Rita Cucchiara, Stan Sclaroff, Giovanni~Maria
      Farinella, Tao Mei, Marco Bertini, Hugo~Jair Escalante, and Roberto Vezzani
      (eds.), \emph{Pattern Recognition. {ICPR} International Workshops and
      Challenges - Virtual Event, January 10-15, 2021, Proceedings, Part {I}},
      volume 12661 of \emph{Lecture Notes in Computer Science}, pp.\  635--646.
      Springer, 2020.
    \newblock \doi{10.1007/978-3-030-68763-2\_48}.
    \newblock URL \url{https://doi.org/10.1007/978-3-030-68763-2\_48}.
    
    \bibitem[Levow(2006)]{DBLP:conf/acl-sighan/Levow06}
    Gina{-}Anne Levow.
    \newblock The third international chinese language processing bakeoff: Word
      segmentation and named entity recognition.
    \newblock In Hwee~Tou Ng and Olivia O.~Y. Kwong (eds.), \emph{Proceedings of
      the Fifth Workshop on Chinese Language Processing, SIGHAN@COLING/ACL 2006,
      Sydney, Australia, July 22-23, 2006}, pp.\  108--117. Association for
      Computational Linguistics, 2006.
    \newblock URL \url{https://aclanthology.org/W06-0115/}.
    
    \bibitem[Li et~al.(2016)Li, Sun, Johnson, Sciaky, Wei, Leaman, Davis,
      Mattingly, Wiegers, and Lu]{DBLP:journals/biodb/LiSJSWLDMWL16}
    Jiao Li, Yueping Sun, Robin~J. Johnson, Daniela Sciaky, Chih{-}Hsuan Wei,
      Robert Leaman, Allan~Peter Davis, Carolyn~J. Mattingly, Thomas~C. Wiegers,
      and Zhiyong Lu.
    \newblock Biocreative {V} {CDR} task corpus: a resource for chemical disease
      relation extraction.
    \newblock \emph{Database J. Biol. Databases Curation}, 2016, 2016.
    \newblock \doi{10.1093/database/baw068}.
    \newblock URL \url{https://doi.org/10.1093/database/baw068}.
    
    \bibitem[Li et~al.(2023{\natexlab{a}})Li, Sun, Tang, Yan, Wu, Huang, and
      Qiu]{li2023codeielargecodegeneration}
    Peng Li, Tianxiang Sun, Qiong Tang, Hang Yan, Yuanbin Wu, Xuanjing Huang, and
      Xipeng Qiu.
    \newblock Codeie: Large code generation models are better few-shot information
      extractors, 2023{\natexlab{a}}.
    \newblock URL \url{https://arxiv.org/abs/2305.05711}.
    
    \bibitem[Li et~al.(2023{\natexlab{b}})Li, Ma, Zhuang, Gu, Su, and
      Chen]{DB-BLINDER}
    Tianle Li, Xueguang Ma, Alex Zhuang, Yu~Gu, Yu~Su, and Wenhu Chen.
    \newblock Few-shot in-context learning on knowledge base question answering.
    \newblock In Anna Rogers, Jordan~L. Boyd{-}Graber, and Naoaki Okazaki (eds.),
      \emph{Proceedings of the 61st Annual Meeting of the Association for
      Computational Linguistics (Volume 1: Long Papers), {ACL} 2023, Toronto,
      Canada, July 9-14, 2023}, pp.\  6966--6980. Association for Computational
      Linguistics, 2023{\natexlab{b}}.
    \newblock \doi{10.18653/v1/2023.acl-long.385}.
    \newblock URL \url{https://doi.org/10.18653/v1/2023.acl-long.385}.
    
    \bibitem[Li et~al.(2025{\natexlab{a}})Li, Dong, Jin, Zhang, Zhou, Zhu, Zhang,
      and Dou]{li2025search}
    Xiaoxi Li, Guanting Dong, Jiajie Jin, Yuyao Zhang, Yujia Zhou, Yutao Zhu,
      Peitian Zhang, and Zhicheng Dou.
    \newblock Search-o1: Agentic search-enhanced large reasoning models.
    \newblock \emph{arXiv preprint arXiv:2501.05366}, 2025{\natexlab{a}}.
    
    \bibitem[Li et~al.(2025{\natexlab{b}})Li, Jin, Dong, Qian, Zhu, Wu, Wen, and
      Dou]{Li2025webthinker}
    Xiaoxi Li, Jiajie Jin, Guanting Dong, Hongjin Qian, Yutao Zhu, Yongkang Wu,
      Ji-Rong Wen, and Zhicheng Dou.
    \newblock Webthinker: Empowering large reasoning models with deep research
      capability.
    \newblock \emph{arXiv preprint arXiv:2504.21776}, 2025{\natexlab{b}}.
    
    \bibitem[Li et~al.(2020)Li, Li, Pan, Chen, Peng, Wang, Lyu, and
      Zhu]{DBLP:conf/nlpcc/LiLPCPWLZ20}
    Xinyu Li, Fayuan Li, Lu~Pan, Yuguang Chen, Weihua Peng, Quan Wang, Yajuan Lyu,
      and Yong Zhu.
    \newblock Duee: {A} large-scale dataset for chinese event extraction in
      real-world scenarios.
    \newblock In Xiaodan Zhu, Min Zhang, Yu~Hong, and Ruifang He (eds.),
      \emph{Natural Language Processing and Chinese Computing - 9th {CCF}
      International Conference, {NLPCC} 2020, Zhengzhou, China, October 14-18,
      2020, Proceedings, Part {II}}, volume 12431 of \emph{Lecture Notes in
      Computer Science}, pp.\  534--545. Springer, 2020.
    \newblock \doi{10.1007/978-3-030-60457-8\_44}.
    \newblock URL \url{https://doi.org/10.1007/978-3-030-60457-8\_44}.
    
    \bibitem[Li et~al.(2024)Li, Zeng, Zuo, Ren, Liu, Su, Guo, Liu, Lixiang, Hu,
      et~al.]{li2024knowcoder}
    Zixuan Li, Yutao Zeng, Yuxin Zuo, Weicheng Ren, Wenxuan Liu, Miao Su, Yucan
      Guo, Yantao Liu, Lixiang Lixiang, Zhilei Hu, et~al.
    \newblock Knowcoder: Coding structured knowledge into llms for universal
      information extraction.
    \newblock In \emph{Proceedings of the 62nd Annual Meeting of the Association
      for Computational Linguistics (Volume 1: Long Papers)}, pp.\  8758--8779,
      2024.
    
    \bibitem[Liu et~al.(2025)Liu, Li, Bai, Zuo, Xu, Jin, Guo, and
      Cheng]{liu2025towards}
    Wenxuan Liu, Zixuan Li, Long Bai, Yuxin Zuo, Daozhu Xu, Xiaolong Jin, Jiafeng
      Guo, and Xueqi Cheng.
    \newblock Towards event extraction with massive types: Llm-based collaborative
      annotation and partitioning extraction.
    \newblock \emph{arXiv preprint arXiv:2503.02628}, 2025.
    
    \bibitem[Liu et~al.(2019)Liu, Meng, Zhang, Xu, Chen, and
      Zhou]{MITReviewDataset}
    Yijin Liu, Fandong Meng, Jinchao Zhang, Jinan Xu, Yufeng Chen, and Jie Zhou.
    \newblock {GCDT:} {A} global context enhanced deep transition architecture for
      sequence labeling.
    \newblock \emph{CoRR}, abs/1906.02437, 2019.
    \newblock URL \url{http://arxiv.org/abs/1906.02437}.
    
    \bibitem[Liu et~al.(2021{\natexlab{a}})Liu, Wang, Gu, Zhang, Zhang, and
      Wang]{liu2021graphine}
    Zequn Liu, Shukai Wang, Yiyang Gu, Ruiyi Zhang, Ming Zhang, and Sheng Wang.
    \newblock Graphine: A dataset for graph-aware terminology definition
      generation.
    \newblock In \emph{Proceedings of the 2021 Conference on Empirical Methods in
      Natural Language Processing}, pp.\  3453--3463, 2021{\natexlab{a}}.
    
    \bibitem[Liu et~al.(2021{\natexlab{b}})Liu, Xu, Wen, Jiang, Wu, and
      Yuan]{liu2021temp}
    Zichen Liu, Hongyuan Xu, Yanlong Wen, Ning Jiang, Haiying Wu, and Xiaojie Yuan.
    \newblock Temp: Taxonomy expansion with dynamic margin loss through
      taxonomy-paths.
    \newblock In \emph{Proceedings of the 2021 Conference on Empirical Methods in
      Natural Language Processing}, pp.\  3854--3863, 2021{\natexlab{b}}.
    
    \bibitem[Luan et~al.(2018{\natexlab{a}})Luan, He, Ostendorf, and
      Hajishirzi]{DBLP:conf/emnlp/LuanHOH18}
    Yi~Luan, Luheng He, Mari Ostendorf, and Hannaneh Hajishirzi.
    \newblock Multi-task identification of entities, relations, and coreference for
      scientific knowledge graph construction.
    \newblock In Ellen Riloff, David Chiang, Julia Hockenmaier, and Jun'ichi Tsujii
      (eds.), \emph{Proceedings of the 2018 Conference on Empirical Methods in
      Natural Language Processing, Brussels, Belgium, October 31 - November 4,
      2018}, pp.\  3219--3232. Association for Computational Linguistics,
      2018{\natexlab{a}}.
    \newblock \doi{10.18653/V1/D18-1360}.
    \newblock URL \url{https://doi.org/10.18653/v1/d18-1360}.
    
    \bibitem[Luan et~al.(2018{\natexlab{b}})Luan, He, Ostendorf, and
      Hajishirzi]{SciERC_DATASET}
    Yi~Luan, Luheng He, Mari Ostendorf, and Hannaneh Hajishirzi.
    \newblock Multi-task identification of entities, relations, and coreference for
      scientific knowledge graph construction, 2018{\natexlab{b}}.
    
    \bibitem[Ma et~al.(2024)Ma, Xu, Jiang, Li, Qu, and Guo]{ma2024think}
    Shengjie Ma, Chengjin Xu, Xuhui Jiang, Muzhi Li, Huaren Qu, and Jian Guo.
    \newblock Think-on-graph 2.0: Deep and interpretable large language model
      reasoning with knowledge graph-guided retrieval.
    \newblock \emph{arXiv e-prints}, pp.\  arXiv--2407, 2024.
    
    \bibitem[Moskvoretskii et~al.(2024)Moskvoretskii, Neminova, Lobanova,
      Panchenko, and Nikishina]{moskvoretskii2024taxollama}
    Viktor Moskvoretskii, Ekaterina Neminova, Alina Lobanova, Alexander Panchenko,
      and Irina Nikishina.
    \newblock Taxollama: Wordnet-based model for solving multiple lexical semantic
      tasks.
    \newblock \emph{arXiv preprint arXiv:2403.09207}, 2024.
    
    \bibitem[Pan et~al.(2017)Pan, Zhang, May, Nothman, Knight, and Ji]{wikiann}
    Xiaoman Pan, Boliang Zhang, Jonathan May, Joel Nothman, Kevin Knight, and Heng
      Ji.
    \newblock Cross-lingual name tagging and linking for 282 languages.
    \newblock In \emph{Proceedings of the 55th Annual Meeting of the Association
      for Computational Linguistics (Volume 1: Long Papers)}, pp.\  1946--1958,
      Vancouver, Canada, July 2017. Association for Computational Linguistics.
    \newblock \doi{10.18653/v1/P17-1178}.
    \newblock URL \url{https://aclanthology.org/P17-1178}.
    
    \bibitem[Pyysalo \& Ananiadou(2014)Pyysalo and
      Ananiadou]{DBLP:journals/bioinformatics/PyysaloA14}
    Sampo Pyysalo and Sophia Ananiadou.
    \newblock Anatomical entity mention recognition at literature scale.
    \newblock \emph{Bioinform.}, 30\penalty0 (6):\penalty0 868--875, 2014.
    \newblock \doi{10.1093/BIOINFORMATICS/BTT580}.
    \newblock URL \url{https://doi.org/10.1093/bioinformatics/btt580}.
    
    \bibitem[Riedel et~al.(2010)Riedel, Yao, and McCallum]{NYT_DATASET}
    Sebastian Riedel, Limin Yao, and Andrew McCallum.
    \newblock Modeling relations and their mentions without labeled text.
    \newblock In \emph{ECML/PKDD}, 2010.
    
    \bibitem[Roth \& Yih(2004)Roth and Yih]{roth-yih-2004-linear}
    Dan Roth and Wen-tau Yih.
    \newblock A linear programming formulation for global inference in natural
      language tasks.
    \newblock In \emph{Proceedings of the Eighth Conference on Computational
      Natural Language Learning ({C}o{NLL}-2004) at {HLT}-{NAACL} 2004}, pp.\
      1--8, Boston, Massachusetts, USA, May 6 - May 7 2004. Association for
      Computational Linguistics.
    \newblock URL \url{https://aclanthology.org/W04-2401}.
    
    \bibitem[Sainz et~al.(2024)Sainz, García-Ferrero, Agerri, de~Lacalle, Rigau,
      and Agirre]{sainz2024gollieannotationguidelinesimprove}
    Oscar Sainz, Iker García-Ferrero, Rodrigo Agerri, Oier~Lopez de~Lacalle,
      German Rigau, and Eneko Agirre.
    \newblock Gollie: Annotation guidelines improve zero-shot
      information-extraction, 2024.
    \newblock URL \url{https://arxiv.org/abs/2310.03668}.
    
    \bibitem[Sang \& Meulder(2003)Sang and Meulder]{conll_2003}
    Erik F. Tjong~Kim Sang and Fien~De Meulder.
    \newblock Introduction to the conll-2003 shared task: Language-independent
      named entity recognition.
    \newblock In Walter Daelemans and Miles Osborne (eds.), \emph{Proceedings of
      the Seventh Conference on Natural Language Learning, CoNLL 2003, Held in
      cooperation with {HLT-NAACL} 2003, Edmonton, Canada, May 31 - June 1, 2003},
      pp.\  142--147. {ACL}, 2003.
    \newblock URL \url{https://aclanthology.org/W03-0419/}.
    
    \bibitem[Satyapanich et~al.(2020)Satyapanich, Ferraro, and
      Finin]{DBLP:conf/aaai/SatyapanichFF20}
    Taneeya Satyapanich, Francis Ferraro, and Tim Finin.
    \newblock {CASIE:} extracting cybersecurity event information from text.
    \newblock In \emph{The Thirty-Fourth {AAAI} Conference on Artificial
      Intelligence, {AAAI} 2020, The Thirty-Second Innovative Applications of
      Artificial Intelligence Conference, {IAAI} 2020, The Tenth {AAAI} Symposium
      on Educational Advances in Artificial Intelligence, {EAAI} 2020, New York,
      NY, USA, February 7-12, 2020}, pp.\  8749--8757. {AAAI} Press, 2020.
    \newblock \doi{10.1609/AAAI.V34I05.6401}.
    \newblock URL \url{https://doi.org/10.1609/aaai.v34i05.6401}.
    
    \bibitem[Shao et~al.(2023)Shao, Gong, Shen, Huang, Duan, and
      Chen]{shao2023enhancing}
    Zhihong Shao, Yeyun Gong, Yelong Shen, Minlie Huang, Nan Duan, and Weizhu Chen.
    \newblock Enhancing retrieval-augmented large language models with iterative
      retrieval-generation synergy.
    \newblock \emph{arXiv preprint arXiv:2305.15294}, 2023.
    
    \bibitem[Shen et~al.(2020)Shen, Shen, Xiong, Wang, Wang, and
      Han]{shen2020taxoexpan}
    Jiaming Shen, Zhihong Shen, Chenyan Xiong, Chi Wang, Kuansan Wang, and Jiawei
      Han.
    \newblock Taxoexpan: Self-supervised taxonomy expansion with position-enhanced
      graph neural network.
    \newblock In \emph{Proceedings of The Web Conference 2020}, pp.\  486--497,
      2020.
    
    \bibitem[Shen et~al.(2024)Shen, Zhang, Zhang, and Han]{shen2024unified}
    Yanzhen Shen, Yu~Zhang, Yunyi Zhang, and Jiawei Han.
    \newblock A unified taxonomy-guided instruction tuning framework for entity set
      expansion and taxonomy expansion.
    \newblock \emph{arXiv preprint arXiv:2402.13405}, 2024.
    
    \bibitem[Shu et~al.(2022)Shu, Yu, Li, Karlsson, Ma, Qu, and Lin]{grailqa1}
    Yiheng Shu, Zhiwei Yu, Yuhan Li, B{\"o}rje Karlsson, Tingting Ma, Yuzhong Qu,
      and Chin-Yew Lin.
    \newblock {TIARA}: Multi-grained retrieval for robust question answering over
      large knowledge base.
    \newblock In \emph{Proceedings of the 2022 Conference on Empirical Methods in
      Natural Language Processing}, pp.\  8108--8121, Abu Dhabi, United Arab
      Emirates, December 2022. Association for Computational Linguistics.
    \newblock \doi{10.18653/v1/2022.emnlp-main.555}.
    \newblock URL \url{https://aclanthology.org/2022.emnlp-main.555}.
    
    \bibitem[Snell et~al.(2024)Snell, Lee, Xu, and Kumar]{snell2024scaling}
    Charlie Snell, Jaehoon Lee, Kelvin Xu, and Aviral Kumar.
    \newblock Scaling llm test-time compute optimally can be more effective than
      scaling model parameters.
    \newblock \emph{arXiv preprint arXiv:2408.03314}, 2024.
    
    \bibitem[Song et~al.(2025)Song, Jiang, Min, Chen, Chen, Zhao, Fang, and
      Wen]{song2025r1}
    Huatong Song, Jinhao Jiang, Yingqian Min, Jie Chen, Zhipeng Chen, Wayne~Xin
      Zhao, Lei Fang, and Ji-Rong Wen.
    \newblock R1-searcher: Incentivizing the search capability in llms via
      reinforcement learning.
    \newblock \emph{arXiv preprint arXiv:2503.05592}, 2025.
    
    \bibitem[Sun et~al.(2023)Sun, Xu, Tang, Wang, Lin, Gong, Ni, Shum, and
      Guo]{sun2023think}
    Jiashuo Sun, Chengjin Xu, Lumingyuan Tang, Saizhuo Wang, Chen Lin, Yeyun Gong,
      Lionel~M Ni, Heung-Yeung Shum, and Jian Guo.
    \newblock Think-on-graph: Deep and responsible reasoning of large language
      model on knowledge graph.
    \newblock \emph{arXiv preprint arXiv:2307.07697}, 2023.
    
    \bibitem[Takeoka et~al.(2021)Takeoka, Akimoto, and Oyamada]{takeoka2021low}
    Kunihiro Takeoka, Kosuke Akimoto, and Masafumi Oyamada.
    \newblock Low-resource taxonomy enrichment with pretrained language models.
    \newblock In \emph{Proceedings of the 2021 Conference on Empirical Methods in
      Natural Language Processing}, pp.\  2747--2758, 2021.
    
    \bibitem[Tedeschi \& Navigli(2022)Tedeschi and Navigli]{multiNERD_DATASET}
    Simone Tedeschi and Roberto Navigli.
    \newblock {M}ulti{NERD}: A multilingual, multi-genre and fine-grained dataset
      for named entity recognition (and disambiguation).
    \newblock In \emph{Findings of the Association for Computational Linguistics:
      NAACL 2022}, pp.\  801--812, Seattle, United States, July 2022. Association
      for Computational Linguistics.
    \newblock \doi{10.18653/v1/2022.findings-naacl.60}.
    \newblock URL \url{https://aclanthology.org/2022.findings-naacl.60}.
    
    \bibitem[Walker et~al.(2006)Walker, Strassel, Medero, and
      Maeda]{ace2005-annotation}
    Christopher Walker, Stephanie Strassel, Julie Medero, and Kazuaki Maeda.
    \newblock Ace 2005 multilingual training corpus, 2006.
    \newblock URL \url{https://catalog.ldc.upenn.edu/LDC2006T06}.
    
    \bibitem[Wang et~al.(2023{\natexlab{a}})Wang, Duan, Wang, Li, Xian, Yin, Rong,
      and Xiong]{wang2023knowledgedriven}
    Keheng Wang, Feiyu Duan, Sirui Wang, Peiguang Li, Yunsen Xian, Chuantao Yin,
      Wenge Rong, and Zhang Xiong.
    \newblock Knowledge-driven cot: Exploring faithful reasoning in llms for
      knowledge-intensive question answering, 2023{\natexlab{a}}.
    
    \bibitem[Wang et~al.(2022)Wang, Zhao, Zheng, and Liu]{wang2022qen}
    Suyuchen Wang, Ruihui Zhao, Yefeng Zheng, and Bang Liu.
    \newblock Qen: Applicable taxonomy completion via evaluating full taxonomic
      relations.
    \newblock In \emph{Proceedings of the ACM Web Conference 2022}, pp.\
      1008--1017, 2022.
    
    \bibitem[Wang et~al.(2023{\natexlab{b}})Wang, Zhou, Zu, Xia, Chen, Zhang,
      Zheng, Ye, Zhang, Gui, Kang, Yang, Li, and
      Du]{wang2023instructuiemultitaskinstructiontuning}
    Xiao Wang, Weikang Zhou, Can Zu, Han Xia, Tianze Chen, Yuansen Zhang, Rui
      Zheng, Junjie Ye, Qi~Zhang, Tao Gui, Jihua Kang, Jingsheng Yang, Siyuan Li,
      and Chunsai Du.
    \newblock Instructuie: Multi-task instruction tuning for unified information
      extraction, 2023{\natexlab{b}}.
    \newblock URL \url{https://arxiv.org/abs/2304.08085}.
    
    \bibitem[Wang et~al.(2023{\natexlab{c}})Wang, Li, and
      Ji]{wang2023code4structcodegenerationfewshot}
    Xingyao Wang, Sha Li, and Heng Ji.
    \newblock Code4struct: Code generation for few-shot event structure prediction,
      2023{\natexlab{c}}.
    \newblock URL \url{https://arxiv.org/abs/2210.12810}.
    
    \bibitem[Wei et~al.(2022)Wei, Wang, Schuurmans, Bosma, Xia, Chi, Le, Zhou,
      et~al.]{wei2022chain}
    Jason Wei, Xuezhi Wang, Dale Schuurmans, Maarten Bosma, Fei Xia, Ed~Chi, Quoc~V
      Le, Denny Zhou, et~al.
    \newblock Chain-of-thought prompting elicits reasoning in large language
      models.
    \newblock \emph{Advances in neural information processing systems},
      35:\penalty0 24824--24837, 2022.
    
    \bibitem[Wu et~al.(2025)Wu, Zhu, and Liu]{wu2025agentic}
    Junde Wu, Jiayuan Zhu, and Yuyuan Liu.
    \newblock Agentic reasoning: Reasoning llms with tools for the deep research.
    \newblock \emph{arXiv preprint arXiv:2502.04644}, 2025.
    
    \bibitem[Xiao et~al.(2024)Xiao, Wang, Xu, Wang, Yang, Wang, Luo, Wang, Mao, and
      Zeng]{xiao2024yayiuiechatenhancedinstructiontuning}
    Xinglin Xiao, Yijie Wang, Nan Xu, Yuqi Wang, Hanxuan Yang, Minzheng Wang, Yin
      Luo, Lei Wang, Wenji Mao, and Daniel Zeng.
    \newblock Yayi-uie: A chat-enhanced instruction tuning framework for universal
      information extraction, 2024.
    \newblock URL \url{https://arxiv.org/abs/2312.15548}.
    
    \bibitem[Xu et~al.(2022)Xu, Chen, Liu, Wen, and Yuan]{xu2022taxoprompt}
    Hongyuan Xu, Yunong Chen, Zichen Liu, Yanlong Wen, and Xiaojie Yuan.
    \newblock Taxoprompt: A prompt-based generation method with taxonomic context
      for self-supervised taxonomy expansion.
    \newblock In \emph{IJCAI}, pp.\  4432--4438, 2022.
    
    \bibitem[Xu et~al.(2024)Xu, Liu, Yan, Wang, Yu, Zeng, Xiao, Liu, Yu, and
      Xiong]{xu2024activerag}
    Zhipeng Xu, Zhenghao Liu, Yukun Yan, Shuo Wang, Shi Yu, Zheni Zeng, Chaojun
      Xiao, Zhiyuan Liu, Ge~Yu, and Chenyan Xiong.
    \newblock Activerag: Autonomously knowledge assimilation and accommodation
      through retrieval-augmented agents.
    \newblock \emph{arXiv preprint arXiv:2402.13547}, 2024.
    
    \bibitem[Yang et~al.(2025)Yang, Zhao, Huang, Ye, Wang, Zheng, Nan, Wang, Xu,
      Huang, Zhang, Gui, Zhang, and
      Huang]{yang2025boundarieslearninguniversalentity}
    Yuming Yang, Wantong Zhao, Caishuang Huang, Junjie Ye, Xiao Wang, Huiyuan
      Zheng, Yang Nan, Yuran Wang, Xueying Xu, Kaixin Huang, Yunke Zhang, Tao Gui,
      Qi~Zhang, and Xuanjing Huang.
    \newblock Beyond boundaries: Learning a universal entity taxonomy across
      datasets and languages for open named entity recognition, 2025.
    \newblock URL \url{https://arxiv.org/abs/2406.11192}.
    
    \bibitem[Yu et~al.(2023)Yu, Zhang, Ng, Zhu, Li, Wang, Hu, Wang, Wang, and
      Xiang]{webqsp1}
    Donghan Yu, Sheng Zhang, Patrick Ng, Henghui Zhu, Alexander~Hanbo Li, Jun Wang,
      Yiqun Hu, William Wang, Zhiguo Wang, and Bing Xiang.
    \newblock Decaf: Joint decoding of answers and logical forms for question
      answering over knowledge bases, 2023.
    
    \bibitem[Yu et~al.(2020)Yu, Li, Shen, Feng, Sun, and Zhang]{yu2020steam}
    Yue Yu, Yinghao Li, Jiaming Shen, Hao Feng, Jimeng Sun, and Chao Zhang.
    \newblock Steam: Self-supervised taxonomy expansion with mini-paths.
    \newblock In \emph{Proceedings of the 26th ACM SIGKDD International Conference
      on Knowledge Discovery \& Data Mining}, pp.\  1026--1035, 2020.
    
    \bibitem[Zeng et~al.(2024)Zeng, Bai, Tan, Wu, Feng, and
      Jiang]{zeng2024codetaxo}
    Qingkai Zeng, Yuyang Bai, Zhaoxuan Tan, Zhenyu Wu, Shangbin Feng, and Meng
      Jiang.
    \newblock Codetaxo: Enhancing taxonomy expansion with limited examples via code
      language prompts.
    \newblock \emph{arXiv preprint arXiv:2408.09070}, 2024.
    
    \bibitem[Zhang \& Yang(2018)Zhang and Yang]{zhang-yang-2018-chinese}
    Yue Zhang and Jie Yang.
    \newblock {C}hinese {NER} using lattice {LSTM}.
    \newblock In \emph{Proceedings of the 56th Annual Meeting of the Association
      for Computational Linguistics (Volume 1: Long Papers)}, pp.\  1554--1564,
      Melbourne, Australia, July 2018. Association for Computational Linguistics.
    \newblock \doi{10.18653/v1/P18-1144}.
    \newblock URL
      \url{[https://aclanthology.org/P18-1144](https://aclanthology.org/P18-1144)}.
    
    \bibitem[Zhao et~al.()Zhao, Zhou, Li, Tang, Wang, Hou, Min, Zhang, Zhang, Dong,
      et~al.]{zhaosurvey}
    Wayne~Xin Zhao, Kun Zhou, Junyi Li, Tianyi Tang, Xiaolei Wang, Yupeng Hou,
      Yingqian Min, Beichen Zhang, Junjie Zhang, Zican Dong, et~al.
    \newblock A survey of large language models.
    
    \bibitem[Zheng et~al.(2024)Zheng, Zhang, Zhang, Ye, Luo, Feng, and
      Ma]{zheng2024llamafactory}
    Yaowei Zheng, Richong Zhang, Junhao Zhang, Yanhan Ye, Zheyan Luo, Zhangchi
      Feng, and Yongqiang Ma.
    \newblock Llamafactory: Unified efficient fine-tuning of 100+ language models.
    \newblock In \emph{Proceedings of the 62nd Annual Meeting of the Association
      for Computational Linguistics (Volume 3: System Demonstrations)}, Bangkok,
      Thailand, 2024. Association for Computational Linguistics.
    \newblock URL \url{http://arxiv.org/abs/2403.13372}.
    
    \bibitem[Zheng et~al.(2025)Zheng, Fu, Hu, Cai, Ye, Lu, and
      Liu]{zheng2025deepresearcher}
    Yuxiang Zheng, Dayuan Fu, Xiangkun Hu, Xiaojie Cai, Lyumanshan Ye, Pengrui Lu,
      and Pengfei Liu.
    \newblock Deepresearcher: Scaling deep research via reinforcement learning in
      real-world environments.
    \newblock \emph{arXiv preprint arXiv:2504.03160}, 2025.
    
    \bibitem[Zhou et~al.(2024)Zhou, Zhang, Gu, Chen, and
      Poon]{zhou2024universalnertargeteddistillationlarge}
    Wenxuan Zhou, Sheng Zhang, Yu~Gu, Muhao Chen, and Hoifung Poon.
    \newblock Universalner: Targeted distillation from large language models for
      open named entity recognition, 2024.
    \newblock URL \url{https://arxiv.org/abs/2308.03279}.
    
    \bibitem[Zhu et~al.(2025)Zhu, Shi, Li, Bai, Jin, Guo, and
      Cheng]{zhu2025towards}
    Jizhao Zhu, Akang Shi, Zixuan Li, Long Bai, Xiaolong Jin, Jiafeng Guo, and
      Xueqi Cheng.
    \newblock Towards robust universal information extraction: Benchmark,
      evaluation, and solution.
    \newblock \emph{arXiv preprint arXiv:2503.03201}, 2025.
    
    \bibitem[Zuo et~al.(2024)Zuo, Jiang, Liu, Li, Bai, Wang, Zeng, Jin, Guo, and
      Cheng]{zuo2024alignxie}
    Yuxin Zuo, Wenxuan Jiang, Wenxuan Liu, Zixuan Li, Long Bai, Hanbin Wang, Yutao
      Zeng, Xiaolong Jin, Jiafeng Guo, and Xueqi Cheng.
    \newblock Alignxie: Improving multilingual information extraction by
      cross-lingual alignment.
    \newblock \emph{arXiv preprint arXiv:2411.04794}, 2024.
    
    \end{thebibliography}
    

==> tables/main.tex <==


\begin{table}[t]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.2}
    \caption{Main results. The best performance is set in bold, and the second best is set in underline.}\label{tab:main}
    \begin{tabular}{lcccccccc}
        \toprule
        \textbf{Method} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{PopQA} & \textbf{HotpotQA} & \textbf{2wiki} & \textbf{Musique} & \textbf{Bamboogle} & \textbf{Avg.} \\
        \midrule
        \multicolumn{8}{l}{\textbf{Qwen2.5-7b-Base/Instruct}} \\
        Direct Inference & 0.134 & 0.408 & 0.140 & 0.183 & 0.250 & 0.031 & 0.120 & 0.181 \\
        CoT & 0.048 & 0.185 & 0.054 & 0.092 & 0.111 & 0.022 & 0.232 & 0.106 \\
        IRCoT & 0.224 & 0.478 & 0.301 & 0.133 & 0.149 & 0.072 & 0.224 & 0.239 \\
        Search-o1 & 0.151 & 0.443 & 0.131 & 0.187 & 0.176 & 0.058 & 0.296 & 0.206 \\
        RAG & 0.349 & \underline{0.585} & 0.392 & 0.299 & 0.235 & 0.058 & 0.208 & 0.304 \\
        SFT & 0.318 & 0.354 & 0.121 & 0.217 & 0.259 & 0.066 & 0.112 & 0.207  \\
        R1-base & 0.297 & 0.539 & 0.202 & 0.242 & 0.273 & 0.083 & 0.296 & 0.276  \\
        R1-instruct & 0.270 & 0.537 & 0.199 & 0.237 & 0.292 & 0.072 & 0.293 & 0.271  \\
        \hdashline
        Search-R1-base & \textbf{0.412} & 0.568 & \textbf{0.428} & \underline{0.356} & \underline{0.322} & \underline{0.142} & \underline{0.384} & \underline{0.373}  \\
        Search-R1-instruct & \underline{0.397} & \textbf{0.606} & \underline{0.404} & \textbf{0.380} & \textbf{0.326} & \textbf{0.168} & \textbf{0.408} & \textbf{0.384} \\
        \midrule
        \multicolumn{8}{l}{\textbf{Qwen2.5-3b-Base/Instruct}} \\
        Direct Inference & 0.106 & 0.288 & 0.108 & 0.149 & 0.244 & 0.020 & 0.024 & 0.134 \\
        CoT & 0.023 & 0.032 & 0.005 & 0.021 & 0.021 & 0.002 & 0.000 & 0.015 \\
        IRCoT & 0.111 & 0.312 & 0.200 & 0.164 & 0.171 & 0.067 & 0.240 & 0.181 \\
        Search-o1 & 0.238 & 0.472 & 0.262 & 0.221 & 0.218 & 0.054 & \textbf{0.320} & 0.255 \\
        RAG & \textbf{0.348} & \textbf{0.544} & \textbf{0.387} & 0.255 & 0.226 & 0.047 & 0.080 & 0.270  \\
        SFT & 0.249 & 0.292 & 0.104 & 0.186 & 0.248 & 0.044 & 0.112 & 0.176  \\
        R1-base & 0.226 & 0.455 & 0.173 & 0.201 & 0.268 & 0.055 & 0.224 & 0.229  \\
        R1-instruct & 0.210 & 0.449 & 0.171 & 0.208 & \underline{0.275} & 0.060 & 0.192 & 0.224  \\
        \hdashline
        Search-R1-base & \underline{0.341} & 0.513 & 0.362 & \underline{0.263} & 0.273 & \underline{0.076} & 0.211 & \underline{0.292}  \\
        Search-R1-instruct & 0.323 & \underline{0.537} & \underline{0.364} & \textbf{0.308} & \textbf{0.336} & \textbf{0.105} & \underline{0.315} & \textbf{0.327}  \\
        \midrule
        \multicolumn{8}{l}{\textbf{LLaMA3.2-3b-Base/Instruct}} \\
        Direct Inference & 0.139 & 0.368 & 0.124 & 0.122 & 0.107 & 0.015 & 0.064 & 0.134 \\
        CoT & 0.246 & 0.487 & 0.166 & 0.051 & 0.083 & 0.006 & 0.024 & 0.152 \\
        IRCoT & 0.363 & 0.566 & \underline{0.428} & 0.238 & 0.236 & 0.072 & 0.208 & 0.301 \\
        Search-o1 & 0.107 & 0.203 & 0.093 & 0.132 & 0.117 & 0.035 & 0.176 & 0.123 \\
        RAG & 0.317 & 0.551 & 0.337 & 0.234 & 0.118 & 0.034 & 0.064 & 0.237  \\
        SFT & 0.320 & 0.341 & 0.122 & 0.206 & 0.257 & 0.064 & 0.120 & 0.204  \\
        R1-base & 0.290 & 0.514 & 0.237 & 0.234 & \textbf{0.279} & 0.055 & 0.146 & 0.251  \\
        R1-instruct & \underline{0.384} & 0.549 & 0.228 & 0.238 & \underline{0.269} & \underline{0.074} & \textbf{0.315} & 0.294 \\
        \hdashline
        Search-R1-base & \textbf{0.394} & \textbf{0.596} & \textbf{0.437} & \underline{0.280} & 0.264 & 0.056 & 0.105 & \underline{0.305}  \\
        Search-R1-instruct & 0.357 & \underline{0.578} & 0.378 & \textbf{0.314} & 0.233 & \textbf{0.090} & \underline{0.306} & \textbf{0.322} \\
        \bottomrule
    \end{tabular}
\end{table}


